Sketch2Human: Deep Human Generation with Disentangled Geometry and Appearance Control

Geometry- and appearance-controlled full-body human image generation is an interesting but challenging task. Existing solutions are either unconditional or dependent on coarse conditions (e.g., pose, text), thus lacking explicit geometry and appearance control of body and garment. Sketching offers such editing ability and has been adopted in various sketch-based face generation and editing solutions. However, directly adapting sketch-based face generation to full-body generation often fails to produce high-fidelity and diverse results due to the high complexity and diversity in the pose, body shape, and garment shape and texture. Recent geometrically controllable diffusion-based methods mainly rely on prompts to generate appearance and it is hard to balance the realism and the faithfulness of their results to the sketch when the input is coarse. This work presents Sketch2Human, the first system for controllable full-body human image generation guided by a semantic sketch (for geometry control) and a reference image (for appearance control). Our solution is based on the latent space of StyleGAN-Human with inverted geometry and appearance latent codes as input. Specifically, we present a sketch encoder trained with a large synthetic dataset sampled from StyleGAN-Human's latent space and directly supervised by sketches rather than real images. Considering the entangled information of partial geometry and texture in StyleGAN-Human and the absence of disentangled datasets, we design a novel training scheme that creates geometry-preserved and appearance-transferred training data to tune a generator to achieve disentangled geometry and appearance control. Although our method is trained with synthetic data, it can handle hand-drawn sketches as well. Qualitative and quantitative evaluations demonstrate the superior performance of our method to state-of-the-art methods.

==> each_part/4_application.tex <==
Due to separate control of geometry and appearance, our system can be applied to various applications. In this section, we present three typical applications.

 \subsection{Sketching Interface for Full-body Human Generation}\label{sec:interface}
 To facilitate the human character design, we design a sketch-based full-body generation user interface (Figure \ref{fig:interface}). Considering that the overall human structure is challenging to draw, especially for novices, we provide geometry guidance in various poses (Figure \ref{fig:interface} (a)). Meanwhile, a list of reference appearance images (pure color and texture) (Figure \ref{fig:interface} (b)) is placed next to (a). The control panel (Figure \ref{fig:interface} (c)) mainly consists of brush colors corresponding to nine semantic parts. When the "Generate" button is pressed, our system generates a synthesized result based on the current sketch and the selected reference appearance image. We also offer an eraser tool for editing the currently drawn sketch. To facilitate the drawing process, our interface operates on Microsoft Surface Pro 4 with a Surface pen to mimic a paper-and-pencil setting. Additionally, our system can produce realistic faces even with simple sketches, and thus it is friendly even for users with little drawing experience.Several results from users can be found in Figure \ref{fig:user}.
 %Several results from users can be found in Figure \ref{fig:user}. Please find more results in the accompanying video.

 \begin{figure}[h]
  \centering
  \includegraphics[width=\linewidth]{figure/interface.pdf}
  \caption{A screenshot of our sketching interface for full-body human generation. The semantic sketch is displayed on the left canvas. The corresponding synthesized result given a selected
  reference appearance image (the orange box in (b)) is displayed on the right. Users might select one of the provided reference sketches (the orange box in (a)) as sketching guidance. 
  The middle buttons (c) allow users to draw and edit according to different semantic components.}
  \label{fig:interface}
\end{figure}



 \subsection{Full-body Geometry and Appearance Editing}
The full-body geometry and appearance editing task aims to change the appearance or geometry (by modifying a corresponding sketch) while preserving its geometry or texture. Benefiting from the full disentanglement between the two aspects, our module enables users to edit from one aspect. 
%(Figure \ref{fig:user}). 
For geometry editing, with the appearance code $w_a$ unchanged and given a series of edited sketch images $\{S_{g,1}, S_{g,2}, \cdots\}$, our method can extract the corresponding geometry code $\{w_{g,1}, w_{g,2}, \cdots\}$ to synthesize edited results via our body generator. Figure \ref{fig:ap_edit} shows the progressive editing sequence by a user.
Our sketch encoder can provide reasonable latent codes for crude or incomplete sketches. This is illustrated through an example involving a coarse-to-fine sketch editing process in Figure \ref{fig:coarse2fine}. Similarly, modifying the appearance code $w_a$ for appearance editing can achieve appearance editing, as shown in Figure \ref{fig:teaser}. The results demonstrate that our proposed method is controllable and can generate high-quality and diverse human images.

\begin{figure}[t]
  \centering
  \includegraphics[width=\linewidth]{figure/application_editing.pdf}
  \caption{\lzf{Application of full-body sketch geometry editing. (a), (b) and (c) respectively consist of the edited semantic sketches and the corresponding results with the same appearance image.}}
  \label{fig:ap_edit}
\end{figure}

\begin{figure*}[h]
  \centering
  \includegraphics[width=0.9\linewidth]{figure/coarse-fine.pdf}
  \caption{\lzf{The coarse-to-fine sketch editing process. For each step in this process, we show the freehand sketch (Left) and the corresponding result (Right).}}
  \label{fig:coarse2fine}
\end{figure*}

\subsection{Full-body Geometry Interpolation}
 Benefiting from the smooth latent space of StyleGAN-Human, our method can produce continuous geometric transformation results from two predefined sketches. With the input of $I_{g,1}$ and $I_{g,2}$, our sketch encoder generates the corresponding geometry codes $w_{g,1}$ and $w_{g,2}$. After mixing each of these two codes with the texture code $w_a$, we can interpolate linearly between the mixed codes $w_{mix8,1}$ and $w_{mix8,2}$.

 \begin{equation}
\label{eq:decoder loss}
\begin{split}
w_{inter} = \alpha \times w_{mix8,1} + (1-\alpha) \times w_{mix8,2}.
\end{split}
\end{equation} 
When $\alpha$ varies between $(0,1)$, our body generator produces the corresponding results. See Figure \ref{fig:inter} for two interpolation examples.
 
 \begin{figure*}
  \centering
  \includegraphics[width=\linewidth]{figure/interpolation.pdf}
  \caption{\lzf{Two examples of full-body geometry interpolation.}} 
  \label{fig:inter}
\end{figure*}
